Sigma terms of the baryon octet in $N_\mathrm{f} = 2+1$ QCD with Wilson quarks

A lot of progress has been made in the direct determination of nucleon sigma terms. Using similar methods, we consider the sigma terms of the other octet baryons as well. These are determined on CLS gauge field ensembles employing the L\"uscher-Weisz gluon action and the Sheikholeslami-Wohlert fermion action with $N_\mathrm{f} = 2 + 1$. The ensembles have pion masses ranging from ${410}\,\mathrm{MeV}$ down to the physical value and lattice spacings covering a range between ${0.098}\,\mathrm{fm}$ and ${0.039}\,\mathrm{fm}$. We present some preliminary results for the pion and strange sigma terms and compare to indirect determinations. To do so, we discuss multi-state fits to tackle the well-known problem of excited state contamination comparing the ratio and summation methods also including priors.

==> backup.tex <==
\begin{figure}
	\begin{center}
		\subfigure[{\footnotesize We obtain $\chi^2/\chi_\mathrm{exp}^2 = 0.6$ and an energy gap of $\Delta \approx 720\, \mathrm {MeV}$.}]{\label{fig:ratio_method}
			\begin{minipage}{1.0\linewidth}
				\centering
				\includegraphics[width=0.45\linewidth]{figs/S400_xi_R_con_UU.pdf}
				\includegraphics[width=0.45\linewidth]{figs/S400_xi_R_con_SS.pdf}
				
				\includegraphics[width=0.45\linewidth]{figs/S400_xi_R_dis_L.pdf}
				\includegraphics[width=0.45\linewidth]{figs/S400_xi_R_dis_S.pdf}
		\end{minipage}}
		\subfigure[{\footnotesize We obtain $\chi^2/\chi_\mathrm{exp}^2 = 0.7$ and an energy gap of $\Delta \approx 745\, \mathrm {MeV}$.}]{\label{fig:summation_method}
			\begin{minipage}{1.0\linewidth}
				\centering
				\includegraphics[width=0.45\linewidth]{figs/S400_xi_R_con_sum_UU.pdf}
				\includegraphics[width=0.45\linewidth]{figs/S400_xi_R_con_sum_SS.pdf}
				
				\includegraphics[width=0.45\linewidth]{figs/S400_xi_R_dis_sum_L.pdf}
				\includegraphics[width=0.45\linewidth]{figs/S400_xi_R_dis_sum_S.pdf}
		\end{minipage}}
	\end{center}
	\caption{{\footnotesize The connected and disconnected ratios that contribute to the sigma terms of the $\Xi$ baryon for ensemble S400: Simultaneous fit to the connected and disconnected ratios is indicated by the coloured shaded regions. The resulting ground state scalar matrix element displayed as a grey band.
			(a) The ratio method is applied to the connected and disconnected contributions. At the top, the connected ratios are plotted against the insertion time $t$ at different source-sink separations $\tf$  for the $\bar{u}u$ current (left) and the $\bar{s}{s}$ current (right). At the bottom, the disconnected ratios are plotted against the source-sink separation $\tf$ at different insertion times $t$ for $J=\bar{l}l$ (left) and $J=\bar{s}s$ (right).
			(b) The summation is now used for the disconnected data so that the bottom row now displays the summed ratios.}}
	\label{fig:ratio_summation_sim_fit}
\end{figure}

==> renormalisation.tex <==
Quark masses $m_q$ are renormalised via  
\begin{align}   
m_q^\mathrm{ren} = \zm   \left[m_q \, + \, (\rmsea - 1) \frac{\Tr M}{\Nf} \right],
\end{align}
which holds up to cut-off effects. $\zm$ is the renormalisation parameter of the non-singlet scalar density and $\Tr M = \Sigma_q m_q$.
The matrix elements must renormalise in the inverse manner w.r.t. the masses so that
\begin{align}
\sigma_{qB}^{\mathrm{ren}} = \left(m_q + (\rmsea-1)\frac{\Tr M}{\Nf} \right) \left(g_{q,S}^B + (\rmsea^{-1}-1)\frac{\Tr g_{S}^B}{\Nf}  \right)
\label{eq:renormalisation}
\end{align}
and $\sigma_{\pi B}^\mathrm{ren} = \sigma_{uB}^\mathrm{ren} + \sigma_{dB}^\mathrm{ren}$. The normalisation factor $\rmsea$ is the ratio of flavour non-singlet and singlet scalar density renormalisation parameters, determined in Refs. \cite{Bali:2016umi,Heitger:2021bmg} for our lattice discretisation. It accounts for the mixing of quark flavours under renormalisation for Wilson fermions.
